Determination of |Vus| from the tau lepton branching fractions

We determine the Cabibbo-Kobayashi-Maskawa matrix (CKM) element |Vus| in several different ways using updated preliminary HFAG averages for the tau lepton branching fractions and we compare the results with the determinations obtained from the kaon decays and from the unitarity of the CKM matrix.

==> papermacros.tex <==
\makeatletter
\DeclareRobustCommand\bfseries{%
  \not@math@alphabet\bfseries\mathbf
  \fontseries\bfdefault\selectfont\boldmath}
\DeclareRobustCommand*{\bm}[1]{%
    \mathchoice{\bmbox{\displaystyle}{#1}}%
               {\bmbox{\textstyle}{#1}}%
               {\bmbox{\scriptstyle}{#1}}%
               {\bmbox{\scriptscriptstyle}{#1}}}
\DeclareRobustCommand*{\bmbox}[2]{\mbox{\bfseries$#1 #2$}}
\makeatother
%%
\makeatletter
%%--- define HFAG tau quantity
\newcommand{\htdef}[2]{%
  \@namedef{hfagtau@#1}{#2}%
}

%%--- retrieve HFAG tau quantity
\newcommand{\htuse}[1]{%
  \ifcsname hfagtau@#1\endcsname
  \@nameuse{hfagtau@#1}\xspace
  \else
  \@latex@error{Undefined name hfagtau@#1}\@eha
  \fi
}

%% \htquantdef{name}{gammaname}{texdescr}{valerr}{val}{err}
\newcommand{\htquantdef}[6]{%
  \ifx&#2&\else
  \@namedef{hfagtau@#1.gn}{\ensuremath{#2}}%
  \fi
  \ifx&#3&\else
  \@namedef{hfagtau@#1.td}{\ensuremath{#3}}%
  \fi
  \ifx&#6&%
    \@namedef{hfagtau@#1}{\ensuremath{#5}}%
  \else
    \ifthenelse{\equal{#6}{0}}{%
      \@namedef{hfagtau@#1}{\ensuremath{#5}}%
    }{%
      \@namedef{hfagtau@#1}{\ensuremath{#4}}%
      \@namedef{hfagtau@#1.v}{\ensuremath{#5}}%
      \@namedef{hfagtau@#1.e}{\ensuremath{#6}}%
    }%
  \fi
}

%% \htmeasdef{name}{quant}{exp}{ref}{valerr}{val}{err}{syst}
\newcommand{\htmeasdef}[8]{%
  \@namedef{hfagtau@#1,quant}{\ensuremath{#2}}%
  \@namedef{hfagtau@#1,exp}{#3}%
  \@namedef{hfagtau@#1,ref}{\cite{#4}}%
  \@namedef{hfagtau@#1}{\ensuremath{#5}}%
  \@namedef{hfagtau@#1,val}{\ensuremath{#6}}%
  \@namedef{hfagtau@#1,stat}{\ensuremath{#7}}%
  \@namedef{hfagtau@#1,syst}{\ensuremath{#8}}%
}

%% \htconstrdef{name}{left}{right}
\newcommand{\htconstrdef}[4]{%
  \@namedef{hfagtau@#1.left}{\ensuremath{#2}}%
  \@namedef{hfagtau@#1.right}{\ensuremath{#3}}%
  \@namedef{hfagtau@#1.right.split}{\ensuremath{#4}}%
  \@namedef{hfagtau@#1.constr.eq}{\htuse{#1.left} ={}& \htuse{#1.right}}%
}

\makeatother

%%
\newcommand{\babar}{\mbox{\slshape B{\smaller A}B{\smaller AR}}\xspace}
%%\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
%%\newcommand{\nub}{\ensuremath{\bar{\nu}}\xspace}
%%
%%--- lepton universality
\newcommand{\lepth}{\ensuremath{L}{}\xspace}%
\newcommand{\leptl}{\ensuremath{\ell}\xspace}%
\newcommand{\opdelta}{\ensuremath{r}}%
%%
\newcommand{\Rhad}{\ensuremath{R_{\text{had}}}\xspace}
\newcommand{\BRhad}{\ensuremath{\BR_{\text{had}}}\xspace}
\newcommand{\Gammahad}{\ensuremath{\Gamma_{\text{had}}}\xspace}
%%\newcommand{\Rstrange}{\ensuremath{R_{\text{strange}}}\xspace}
\newcommand{\Rstrange}{\ensuremath{R_s}\xspace}
\newcommand{\BRstrange}{\ensuremath{\BR_s}\xspace}
\newcommand{\Gammastrange}{\ensuremath{\Gamma_s}\xspace}
\newcommand{\Rnonstrange}{\ensuremath{R_{\text{VA}}}\xspace}
\newcommand{\BRnonstrange}{\ensuremath{\BR_{\text{VA}}}\xspace}
\newcommand{\Gammanonstrange}{\ensuremath{\Gamma_{\text{VA}}}\xspace}
\newcommand{\tauknu}{\ensuremath{\tau^{-} \to K^{-} \nut}\xspace}
\newcommand{\taupinu}{\ensuremath{\tau^{-} \to \pi^{-} \nut}\xspace}
\newcommand{\BFtautoknu}{\ensuremath{\BR(\tauknu)}\xspace}
\newcommand{\BFtautopinu}{\ensuremath{\BR(\taupinu)}\xspace}
\newcommand{\Vud}{\ensuremath{|V_{ud}|}\xspace}
\newcommand{\Vus}{\ensuremath{|V_{us}|}\xspace}
\newcommand{\Vub}{\ensuremath{|V_{ub}|}\xspace}
\newcommand{\VusUni}{\ensuremath{\Vus_{\text{uni}}}\xspace}
\newcommand{\VusTauIncl}{\ensuremath{\Vus_{\tau s}}\xspace}
\newcommand{\VusTauKpi}{\ensuremath{\Vus_{\tau K/\pi}}\xspace}
\newcommand{\VusTauKnu}{\ensuremath{\Vus_{\tau K}}\xspace}
\newcommand{\VusTauKPinu}{\ensuremath{\Vus_{\tau K\pi}}\xspace}
\newcommand{\fpKpi}{\ensuremath{f_+^{K\pi}(0)}\xspace}
\newcommand{\dEM}[1]{\ensuremath{\delta_{\rm EM}^{#1}}\xspace}
\newcommand{\tdSU}[1]{\ensuremath{\tilde{\delta}_{\rm SU(2)}^{#1}}}
%%
\newcommand{\hfagtau}{HFAG-Tau\xspace}
%%
\def\electron   {\ensuremath{e}\xspace}
\def\en         {\ensuremath{e^-}\xspace}   % electron negative (\em is taken)
\let\emi\en
\def\ep         {\ensuremath{e^+}\xspace}
\def\epm        {\ensuremath{e^\pm}\xspace} 
\def\epem       {\ensuremath{e^+e^-}\xspace}
\def\ee         {\ensuremath{e^-e^-}\xspace}
\def\mmu        {\ensuremath{\mu}\xspace}
\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mun        {\ensuremath{\mu^-}\xspace}    % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\mu^+\mu^-}\xspace}
\def\mtau       {\ensuremath{\tau}\xspace}
\def\taup       {\ensuremath{\tau^+}\xspace}
\def\taum       {\ensuremath{\tau^-}\xspace}
\def\tautau     {\ensuremath{\tau^+\tau^-}\xspace}
\def\ellm       {\ensuremath{\ell^-}\xspace}
\def\ellp       {\ensuremath{\ell^+}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nue        {\ensuremath{\nu_e}\xspace}
\def\nueb       {\ensuremath{\nub_e}\xspace}
\def\nuenueb    {\ensuremath{\nue\nueb}\xspace}
\def\num        {\ensuremath{\nu_\mu}\xspace}
\def\numb       {\ensuremath{\nub_\mu}\xspace}
\def\numnumb    {\ensuremath{\num\numb}\xspace}
\def\nut        {\ensuremath{\nu_\tau}\xspace}
\def\nutb       {\ensuremath{\nub_\tau}\xspace}
\def\nutnutb    {\ensuremath{\nut\nutb}\xspace}
\def\nul        {\ensuremath{\nu_\ell}\xspace}
\def\nulb       {\ensuremath{\nub_\ell}\xspace}
\def\nulnulb    {\ensuremath{\nul\nulb}\xspace}

\newcommand{\tev}{\ensuremath{\mathrm{Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{Me\kern -0.1em V\!/}c^2}}\xspace}

